Data Structures for Finite Downsets of Natural Vectors: Theory and Practice

Manipulating downward-closed sets of vectors forms the basis of so-called antichain-based algorithms in verification. In that context, the dimension of the vectors is intimately tied to the size of the input structure to be verified. In this work, we formally analyze the complexity of classical list-based algorithms to manipulate antichains as well as that of Zampuni\'eris's sharing trees and traditional and novel kdtree-based antichain algorithms. In contrast to the existing literature, and to better address the needs of formal verification, our analysis of \kdtree algorithms does not assume that the dimension of the vectors is fixed. Our theoretical results show that kdtrees are asymptotically better than both list- and sharing-tree-based algorithms, as an antichain data structure, when the antichains become exponentially larger than the dimension of the vectors. We evaluate this on applications in the synthesis of reactive systems from linear-temporal logic and parity-objective specifications, and establish empirically that current benchmarks for these computational tasks do not lead to a favorable situation for current implementations of kdtrees.

==> average.tex <==

\section{Average case}

Here onwards, $d$ is the dimension, $n$ is the number of vectors in the antichain and $\ell-1$ is the largest number allowed in the antichain.

$[\ell]^d$ represents the $d$-dimensional lattice, where $[\ell]$ represents the set $\Set{0,\dots,\ell-1}$.

$\alpha(d,\ell)$ is the \emph{width} of the antichain, that is, the maximal size of an antichain in $[\ell]^d$.

$A(d,\ell,n)$ is the total number of antichains in $[\ell]^d$ with exactly $n$ vectors.

$A(d,\ell)$ is the total number of antichains in $[\ell]^d$. 

\[
A(d,\ell)=\sum_{n=1}^{\alpha(d,\ell)}A(d,\ell,n).
\]

Bounds for $A(d,\ell)$ using $\alpha(d,\ell)$ are known \cite{falgasravry2023dedekinds}:

\[
\alpha(d,\ell)\leq\log_2 A(d,\ell)\leq \Big(1+c\cdot\frac{(\log d)^3}{d}\Big)\cdot\alpha(d,\ell).
\]

The lower bound is easy to see, since all the $2^{\alpha(d,\ell)}$ subsets of a maximal antichain are also antichains. 

We are also interested in ``good'' antichains in $[\ell]^d$, that is, antichains such that all the numbers in the same dimension are distinct. $\alpha_G(d,\ell)$, $A_G(d,\ell,n)$ and $A_G(d,\ell)$ are defined analogously for good antichains. It is easy to see $\alpha_G(d,\ell)=\ell$ for $d\geq2$ since there are only $\ell$ unique numbers that can occur in one dimension in a good antichain.

\subsection{$d=2$}

In two dimensions, we have the property that any two vectors in an antichain, say $(p,q)$ and $(r,s)$ must have the property that $p\neq r$, $q\neq s$ and $p>r$ iff $q<s$. Thus, for a given $n\leq\ell$, any two sequences of numbers $0\leq p_1<p_2<\dots<p_n<\ell$ and $\ell>q_1>q_2>\dots>q_n\geq0$ induce an antichain $(p_1,q_1),\dots,(p_n,q_n)$ and all antichains in $[\ell]^2$ can be written in this form. This gives us the following:
\begin{align}
    A(d,\ell,n)&=\binom{\ell}{n}^2,\\
    A(d,\ell)&=\sum_{n=0}^{\ell}A(d,\ell,n)=\sum_{n=0}^{\ell}\binom{\ell}{n}^2=\binom{2\ell}{\ell}.
\end{align}

The last equality follows from the fact that choosing $\ell$ items from $2\ell$ items is the same as choosing $n$ and $\ell-n$ items respectively from two sets containing $\ell$ items. 

Note that all antichains in two dimensions are good, which gives us $A_G(d,\ell,n)=A(d,\ell,n)$ and $A_G(d,\ell)=A(d,\ell)$.

We also have $\alpha(d,\ell)=\ell$ since it is not possible to find sequences of numbers between $0$ and $\ell-1$ of length more than $\ell$ and sequences of length $\ell$ exist.

\subsection{$d\geq3$}

The analysis for higher dimensions is not so trivial. We only provide bounds which help with our average case analysis of the performance of $kd$-trees.\shrisha{hopefully}

How big is $\alpha(d,\ell)$? To give an upper bound, we use the fact that for all $0\leq k\leq\ell-1$, all vectors $x=(x_1,\dots,x_d)$ with $x_1+\dots+x_d=k$ form an antichain. This is easy to see, since for two distinct vectors with the same sum, there must be two components $1\leq m,n\leq d$ such that the component $m$ of one vector is greater than that of the other, and the opposite holds for component $n$. Thus, we are interested in the number of points whose components add to $k$, with the restriction that each component is at most $\ell$.

We conjecture that this number is maximized when $k=\lfloor\frac{\ell d}{2}\rfloor$.
\begin{theorem}[Conjecture]
    The length of the longest antichain in the hypercube $[\ell]^d$ is the same as the size of the set of all points in $[\ell]^d$ such that the sum of all the components of each point is exactly $\lfloor\frac{\ell d}{2}\rfloor$.
\end{theorem}
We will show that the above holds if the following holds:
\begin{proposition}
    For all $n<\lfloor\frac{\ell d}{2}\rfloor$ There is a surjective mapping $f$ from the set of all points which add up to $n$ to those that add up to $n+1$ such that the mapping preserves the following: $f(u)=v$ implies $v>u$.
\end{proposition}

First, we show that the number of points that add to $n$ in $[\ell]^d$ is at most those that add up to $n+1$ for $n<\lfloor\frac{\ell d}{2}\rfloor$. To show this, we first notice the following:

\begin{lemma}
    
\end{lemma}

